Optimization of Epsilon-Greedy Exploration

Modern recommendation systems rely on exploration to learn user preferences for new items, typically implementing uniform exploration policies (e.g., epsilon-greedy) due to their simplicity and compatibility with machine learning (ML) personalization models. Within these systems, a crucial consideration is the rate of exploration - what fraction of user traffic should receive random item recommendations and how this should evolve over time. While various heuristics exist for navigating the resulting exploration-exploitation tradeoff, selecting optimal exploration rates is complicated by practical constraints including batched updates, time-varying user traffic, short time horizons, and minimum exploration requirements. In this work, we propose a principled framework for determining the exploration schedule based on directly minimizing Bayesian regret through stochastic gradient descent (SGD), allowing for dynamic exploration rate adjustment via Model-Predictive Control (MPC). Through extensive experiments with recommendation datasets, we demonstrate that variations in the batch size across periods significantly influence the optimal exploration strategy. Our optimization methods automatically calibrate exploration to the specific problem setting, consistently matching or outperforming the best heuristic for each setting.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\begin{table*}[t]
\scriptsize

$K = 5$ items 
\vspace{0.1cm}

\begin{tabular}{lcccccc|cccccc}
\toprule
 & \multicolumn{6}{c|}{MovieLens-1M} & \multicolumn{6}{c}{Netflix} \\
\midrule
$N$ samples & \multicolumn{3}{c}{500} & \multicolumn{3}{c|}{5000} & \multicolumn{3}{c}{500} & \multicolumn{3}{c}{5000} \\
\midrule
Arrival $\lambda$ & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike \\
\midrule
% \textsf{EpsGreedy}$^{*}$ & 0.278 & 0.309 & 0.332 & 0.145 & 0.154 & 0.157 & 0.121 & 0.128 & 0.143 & 0.065 & 0.072 & 0.072 \\
% \textsf{TheoryETC}$^{*}$ & 0.185 & 0.156 & 0.149 & 0.097 & 0.048 & 0.071 & 0.080 & 0.093 & 0.098 & 0.045 & 0.039 & 0.045 \\
% \textsf{SimpleETC}       & 0.139 & 0.292 & 0.185 & 0.074 & 0.049 & 0.057 & 0.105 & 0.147 & 0.095 & 0.040 & 0.047 & 0.031 \\
% \midrule
% \textsf{Planner}         & 0.141 & 0.251 & 0.184 & 0.074 & 0.049 & 0.057 & 0.105 & 0.091 & 0.095 & 0.040 & 0.042 & 0.031 \\
% \textsf{Planner (noisy)} & 0.136 & 0.185 & 0.187 & 0.074 & 0.051 & 0.057 & 0.107 & 0.083 & 0.097 & 0.040 & 0.044 & 0.031 \\
% \textsf{MPC}             & 0.131 & 0.164 & 0.168 & 0.074 & 0.045 & 0.056 & 0.095 & 0.084 & 0.081 & 0.037 & 0.033 & 0.029 \\
% \textsf{MPC (noisy)}     & 0.131 & 0.160 & 0.167 & 0.074 & 0.037 & 0.053 & 0.087 & 0.088 & 0.080 & 0.036 & 0.031 & 0.030 \\
% \textsf{TS}              & 0.253 & 0.287 & 0.351 & 0.178 & 0.189 & 0.258&  0.101 & 0.113 & 0.134 & 0.053 & 0.061 & 0.097\\
% \bottomrule
\textsf{EpsGreedy}$^{*}$ & 0.278 & 0.309 & 0.332 & 0.145 & 0.154 & 0.157 & 0.121 & 0.128 & 0.143 & 0.065 & 0.072 & 0.072 \\
\textsf{TheoryETC}$^{*}$ & 0.185 & \textbf{0.156} & \textbf{0.149} & 0.097 & 0.048 & 0.071 & \textbf{0.080} & 0.093 & 0.098 & 0.045 & 0.039 & 0.045 \\
\textsf{SimpleETC}       & 0.139 & 0.292 & 0.185 & \textbf{0.074} & 0.049 & \textbf{0.057} & 0.105 & 0.147 & 0.095 & \textbf{0.040} & 0.047 & \textbf{0.031} \\
\midrule
\textsf{Planner}         & 0.141 & 0.251 & 0.184 & \textbf{0.074} & 0.049 & \textbf{0.057} & 0.105 & 0.091 & 0.095 & \textbf{0.040} & 0.042 & \textbf{0.031} \\
\textsf{Planner (noisy)} & 0.136 & 0.185 & 0.187 & \textbf{0.074} & 0.051 & \textbf{0.057} & 0.107 & \textbf{0.083} & 0.097 & \textbf{0.040} & 0.044 & \textbf{0.031} \\
\textsf{MPC}             & \textbf{0.131} & 0.164 & 0.168 & \textbf{0.074} & 0.045 & \textbf{0.056} & 0.095 & \textbf{0.084} & \textbf{0.081} & \textbf{0.037} & \textbf{0.033} & \textbf{0.029} \\
\textsf{MPC (noisy)}     & \textbf{0.131} & \textbf{0.160} & 0.167 & \textbf{0.074} & \textbf{0.037} & \textbf{0.053} & 0.087 & 0.088 & \textbf{0.080} & \textbf{0.036} & \textbf{0.031} & \textbf{0.030} \\
\midrule
\textsf{TS}              & 0.253 & 0.287 & 0.351 & 0.178 & 0.189 & 0.258 & 0.101 & 0.113 & 0.134 & 0.053 & 0.061 & 0.097 \\
\bottomrule
\end{tabular}

\vspace{0.3cm}
$K = 10$ items 
\vspace{0.1cm}

\begin{tabular}{lcccccc|cccccc}
\toprule
& \multicolumn{6}{c|}{MovieLens-1M} & \multicolumn{6}{c}{Netflix} \\
\midrule
$N$ samples & \multicolumn{3}{c}{500} & \multicolumn{3}{c|}{5000} & \multicolumn{3}{c}{500} & \multicolumn{3}{c}{5000} \\
\midrule
Arrival $\lambda$ & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike \\
\midrule
% \textsf{EpsGreedy}$^{*}$ & 0.455 & 0.496 & 0.511 & 0.227 & 0.232 & 0.266 & 0.196 & 0.226 & 0.243 & 0.127 & 0.132 & 0.144 \\
% \textsf{TheoryETC}$^{*}$ & 0.350 & 0.347 & 0.364 & 0.156 & 0.126 & 0.117 & 0.168 & 0.164 & 0.167 & 0.073 & 0.082 & 0.082 \\
% \textsf{SimpleETC}       & 0.266 & 0.625 & 0.313 & 0.114 & 0.141 & 0.095 & 0.166 & 0.259 & 0.190 & 0.062 & 0.145 & 0.078 \\
% \midrule
% \textsf{Planner}         & 0.265 & 0.387 & 0.313 & 0.114 & 0.145 & 0.095 & 0.165 & 0.162 & 0.193 & 0.062 & 0.144 & 0.078 \\
% \textsf{Planner (noisy)} & 0.255 & 0.368 & 0.324 & 0.114 & 0.137 & 0.095 & 0.164 & 0.172 & 0.181 & 0.062 & 0.130 & 0.078 \\
% \textsf{MPC}             & 0.263 & 0.320 & 0.292 & 0.115 & 0.113 & 0.093 & 0.161 & 0.157 & 0.154 & 0.061 & 0.090 & 0.078 \\
% \textsf{MPC (noisy)}     & 0.272 & 0.361 & 0.291 & 0.113 & 0.126 & 0.084 & 0.156 & 0.152 & 0.160 & 0.061 & 0.081 & 0.076 \\
% \midrule
% \textsf{TS}              & 0.462 & 0.547 & 0.651 & 0.312 & 0.327 & 0.404 & 0.204 & 0.251 & 0.247 & 0.111 & 0.124 & 0.197\\
% \bottomrule
\textsf{EpsGreedy}$^{*}$ & 0.455 & 0.496 & 0.511 & 0.227 & 0.232 & 0.266 & 0.196 & 0.226 & 0.243 & 0.127 & 0.132 & 0.144 \\
\textsf{TheoryETC}$^{*}$ & 0.320 & 0.346 & \textbf{0.292} & 0.155 & 0.126 & 0.117 & 0.168 & 0.164 & 0.167 & 0.073 & \textbf{0.082} & 0.082 \\
\textsf{SimpleETC}       & 0.266 & 0.625 & 0.313 & \textbf{0.114} & 0.141 & 0.095 & 0.166 & 0.259 & 0.190 & \textbf{0.062} & 0.145 & \textbf{0.078} \\
\midrule
\textsf{Planner}         & 0.265 & 0.387 & 0.313 & \textbf{0.114} & 0.145 & 0.095 & 0.165 & 0.162 & 0.193 & \textbf{0.062} & 0.144 & \textbf{0.078} \\
\textsf{Planner (noisy)} & \textbf{0.255} & 0.368 & 0.324 & \textbf{0.114} & 0.137 & 0.095 & 0.164 & 0.172 & 0.181 & \textbf{0.062} & 0.130 & \textbf{0.078} \\
\textsf{MPC}             & 0.263 & \textbf{0.320} & \textbf{0.292} & \textbf{0.115} & \textbf{0.113} & 0.093 & 0.161 & 0.157 & \textbf{0.154} & \textbf{0.061} & 0.090 & \textbf{0.078} \\
\textsf{MPC (noisy)}     & 0.272 & 0.361 & \textbf{0.291} & \textbf{0.113} & 0.126 & \textbf{0.084} & \textbf{0.156} & \textbf{0.152} & 0.160 & \textbf{0.061} & \textbf{0.081} & \textbf{0.076} \\
\midrule
\textsf{TS}              & 0.462 & 0.547 & 0.651 & 0.312 & 0.327 & 0.404 & 0.204 & 0.251 & 0.247 & 0.111 & 0.124 & 0.197 \\
\bottomrule
\end{tabular}

\vspace{0.3cm}
$K = 15$ items 
\vspace{0.1cm}

\begin{tabular}{lcccccc|cccccc}
\toprule
& \multicolumn{6}{c|}{MovieLens-1M} & \multicolumn{6}{c}{Netflix} \\
\midrule
$N$ samples & \multicolumn{3}{c}{500} & \multicolumn{3}{c|}{5000} & \multicolumn{3}{c}{500} & \multicolumn{3}{c}{5000} \\
\midrule
Arrival $\lambda$ & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike \\
\midrule
% best\_eps             & 0.588 & 0.595 & 0.623 & 0.285 & 0.301 & 0.346 & 0.336 & 0.333 & 0.346 & 0.186 & 0.194 & 0.219 \\
% best\_theory\_d       & 0.433 & 0.444 & 0.471 & 0.185 & 0.194 & 0.207 & 0.237 & 0.233 & 0.260 & 0.090 & 0.104 & 0.114 \\
% simple\_etc           & 0.308 & 0.692 & 0.523 & 0.145 & 0.169 & 0.124 & 0.328 & 0.417 & 0.310 & 0.085 & 0.232 & 0.099 \\
% opt\_static\_etc      & 0.308 & 0.402 & 0.523 & 0.145 & 0.165 & 0.124 & 0.328 & 0.307 & 0.310 & 0.085 & 0.232 & 0.099 \\
% est\_opt\_static\_etc & 0.315 & 0.425 & 0.501 & 0.145 & 0.167 & 0.124 & 0.327 & 0.302 & 0.306 & 0.085 & 0.230 & 0.099 \\
% planner               & 0.309 & 0.460 & 0.469 & 0.145 & 0.148 & 0.124 & 0.286 & 0.240 & 0.227 & 0.085 & 0.157 & 0.099 \\
% est\_planner          & 0.308 & 0.455 & 0.478 & 0.145 & 0.154 & 0.124 & 0.296 & 0.231 & 0.230 & 0.082 & 0.163 & 0.099 \\
% \textsf{TS}           & 0.525 & 0.615 & 0.660 & 0.278 & 0.306 & 0.360 & 0.290 & 0.328 & 0.404 & 0.209 & 0.219 & 0.259 \\
\textsf{EpsGreedy}$^{*}$ & 0.588 & 0.595 & 0.623 & 0.285 & 0.301 & 0.346 & 0.336 & 0.333 & 0.346 & 0.186 & 0.194 & 0.219 \\
\textsf{TheoryETC}$^{*}$ & 0.433 & 0.444 & \textbf{0.471} & 0.185 & 0.194 & 0.207 & \textbf{0.237} & \textbf{0.233} & 0.260 & 0.090 & \textbf{0.104} & 0.114 \\
\textsf{SimpleETC}       & \textbf{0.308} & 0.692 & 0.523 & \textbf{0.145} & 0.169 & \textbf{0.124} & 0.328 & 0.417 & 0.310 & \textbf{0.085} & 0.232 & \textbf{0.099} \\
\midrule
\textsf{Planner}         & \textbf{0.308} & \textbf{0.402} & 0.523 & \textbf{0.145} & 0.165 & \textbf{0.124} & 0.328 & 0.307 & 0.310 & \textbf{0.085} & 0.232 & \textbf{0.099} \\
\textsf{Planner (noisy)} & 0.315 & 0.425 & 0.501 & \textbf{0.145} & 0.167 & \textbf{0.124} & 0.327 & 0.302 & 0.306 & \textbf{0.085} & 0.230 & \textbf{0.099} \\
\textsf{MPC}             & \textbf{0.309} & 0.460 & \textbf{0.469} & \textbf{0.145} & \textbf{0.148} & \textbf{0.124} & 0.286 & 0.240 & \textbf{0.227} & \textbf{0.085} & 0.157 & \textbf{0.099} \\
\textsf{MPC (noisy)}     & \textbf{0.308} & 0.455 & 0.478 & \textbf{0.145} & 0.154 & \textbf{0.124} & 0.296 & \textbf{0.231} & \textbf{0.230} & \textbf{0.082} & 0.163 & \textbf{0.099} \\
\midrule
\textsf{TS}              & 0.525 & 0.615 & 0.660 & 0.278 & 0.306 & 0.360 & 0.290 & 0.328 & 0.404 & 0.209 & 0.219 & 0.259 \\
\bottomrule
\end{tabular}

\caption{\label{table:experiments} Average regret across contextual bandit settings. Each cell is averaged over 1000 bandit problems; standard errors are all close to $0.002$. While strategies like \textsf{TheoryETC}$^{*}$ or \textsf{SimpleETC} are good in some situations and poor in others, \textsf{Planner} and \textsf{MPC} match performance or even outperform uniformly across most scenarios, even under noisy estimates of batch sizes.}
\end{table*}

In this section, we investigate whether optimizing the objective in regret produces effective exploration schedules.

\paragraph{Bandit Environment}
To benchmark exploration strategies, we use two datasets to construct realistic contextual bandit problems that model cold-start exploration in recommendation systems
\begin{itemize}
\item \textbf{Movie-Lens 1 Million data} (\emph{ML-1M}): consists of 6,000 users, 4,000 movies, and 1M interactions.
\item \textbf{Netflix Prize data} (\emph{Netflix}): we filter users and movies with less than 100 interactions, leaving with 28,604 users, 9,275 movies, and 3M interactions.
\end{itemize}

In a similar approach to~\cite{liang2022local}, we construct contextual bandit instances by first training a matrix factorization model~\cite{koren2009matrix} (embedding dimension $d=128$) on the data. We train the model to predict the rating, which we use as our reward metric.
% \[
% \min_{x,\theta} \sum_{(i,a) \in \mathcal{D}}\|x_{i}^{\top}\theta_{a} - \text{rating}_{i,a}\|^{2} + \lambda \|x\|_{F}^{2} + \mu \|\theta\|_{F}^{2}
% \]
% for $\lambda = \mu = 1$. 
We use the resulting user embeddings $x_{i}$ and item embeddings $\theta_{a}$ as the ground-truth reward model $r(x_{i},a)=x_{i}^\top \theta_{a}$. For each bandit instance, we randomly select a subset of $K \in \{5, 10, 15\}$ items from the total item set as the item set for the instance, denoted as $\mathcal{A}$. We run the contextual bandit policy for the time horizon of $T$ steps, starting from initial item embedding estimates of $\hat{\theta} = \mathbf{0} \in \R^{Kd}$ for the items in $\mathcal{A}$. At each period $t$, we sample a batch of $n_{t}$ users uniformly at random from the dataset. For a given user embedding $X_{i}$ and an item sampled by the policy $A_{i}$, we generate noisy rewards from the reward model $R_{i,a}=r(X_{i},A_{i}) + \eta_{i}$, where $\eta_{i} \sim N(0,1)$.

In order to assess the impact of batched feedback, we consider different patterns for the batch arrivals. We let $\lambda_{t}$ denote the fraction of users that arrive on period $t$, and we consider the following arrival patterns:
\begin{align*}
    \text{Increasing: } \lambda_{t} &= [2\%, 18\%, 20\%, 20\%, 20\%, 20\%] \\
    \text{Spike: }\lambda_{t} &= [5\%, 35\%, 20\%, 20\%, 20\%] \\
    \text{Constant: }\lambda_{t} &= 10\%\cdot \mathbf{1}_{10} 
\end{align*}
These patterns are motivated by user impressions in online platforms, which may experience predictable spikes (e.g. in the beginning of a new item launch) or may increase over time.
To generate random arrivals, we draw $n_{t} \sim \text{Bin}(N,\lambda_{t})$, where we consider $N \in \{500, 5000\}$. All the algorithms we benchmark do not know the realizations of $n_{t}$, but know $N$ and $\lambda_{t}$. For each choice of $K$, $N$, and arrival pattern $\lambda$, we run 1000 bandit problems, randomly sampling items and batch sizes $n_{t}$ each time, and report the regret~\eqref{eqn:regret} averaged across all problems.

\paragraph{Bandit Policies}

As discussed before, we focus on determining the exploration schedule for uniform exploration policies. Recall that these policies assign an item $a$ to a user $X_{i}$ according to,
\[
\label{eqn:uniform_policy}
\pi_{t}(a|X_{i}) =
\begin{cases}
1/K & \text{w.p. }  \eps_{t} \\
\mathbf{1}
\{
a = \arg \max_{a} X_{i}^{\top}\hat{\theta}_{t,a}
\}
& \text{w.p. } 1- \eps_{t}
\end{cases}
\]
where $\hat{\theta}_{t,a}$ is the Ridge regression estimator of $\theta_{a}$
\[
\hat{\theta}_{t,a} = \arg\min_{\theta \in \R^{d}} \|R_{t-1,a} - X_{t-1,a}\theta\|_{2}^{2} + \nu \|\theta\|_{2}^{2}
\]
where $\nu =1$ is the regularization factor,  $X_{t-1,a}$ is the matrix of all user-embeddings assigned $a$ before period $t$ and $R_{t-1,a}$ is the corresponding vector of observed rewards. Note that $\hat{\theta}_{t,a}$ is only estimated from users in the explore group, but we found that the results didn't qualitatively change if we included data from the exploit group as well. The evaluation metric is regret compared to the oracle optimal policy that assigns user $i$ the item $\arg \max_{a\in \mathcal{A}} r(X_{i},a)$.

We now discuss the exploration strategies we benchmark for choosing the exploration rates $\eps_{t}$.
\begin{itemize}
\item \textbf{Epsilon-Greedy} [$\textsf{EpsGreedy}^{*}$]: constant exploration $\eps_{t} = \eps \in [0,1]$. Performance depends sensitively on $\eps$ so we report the regret of \emph{best} $\eps \in [0.05, 0.01, 0.1, 0.5, 1.0]$ for each problem instance (which is different across instances). This is a strong benchmark that is unrealistic to implement in practice, as it requires already knowing the optimal choice of $\eps$.
\item \textbf{Explore-then-Commit (ETC)} with budget $B = O(d^{2/3}N^{2/3})$ 
 [$\textsf{TheoryETC}^{*}$]. A theoretical recommendation for ETC is to use a budget of order $O(d^{1/3}N^{2/3})$~\cite{langford2007epoch, li2022simple, hao2020high}, and under mild assumptions, this results in a regret scaling of $O(N^{2/3})$. However, setting $B = d^{1/3}N^{2/3}$ tends to explore too much, so instead we report the regret for $B = cd^{1/3}N^{2/3}$ for the \emph{best} constant $c \in [0.05, 0.01, 0.1, 0.5, 1.0]$ (which is different across instances). This benchmark is also unrealistic to use in practice, as it requires already knowing the optimal $c$.
 \item \textbf{Simple ETC} [$\textsf{SimpleETC}^{*}$]: sets $\eps_{1} = 1$ and $\eps_{t} = 0$ for $t > 1$. Despite its simplicity, it is a commonly used heuristic.
 \end{itemize}

We propose the following exploration strategies based on optimization, and propose variants that test the robustness of these algorithms to errors in the input. 
\begin{itemize}
 \item \textbf{Optimization Planner} [$\textsf{Planner}$]: Obtains the schedule via $\eps^{*}_{1:T} =\arg \min_{\eps_{1:T}} \overline{J}_{1}(\eps_{1:T},\beta_{1},\Sigma_{1})$ under (mis-specified) prior $\beta_{1} = \mathbf{0},\Sigma_{1} = I$. Obtains samples of $X_{i}$ from the first batch and uses the batch sizes $\bar{n}_{t} = N\lambda_{t}$ as inputs.
 \item \textbf{Optimization Planner (Noisy)} [$\textsf{Planner (noisy)}$]: Same as $\textsf{Planner}$ but uses noisy predictions of arrival rates $\widehat{n}_{t}=N\hat{\lambda}_{t}$ where $\hat{\lambda}_{t} \sim \text{Dirichlet}_{K\lambda}(\cdot)$ drawn from a Dirichlet distribution with parameter $(K\lambda_{1},...,K\lambda_{T})$.
 \item \textbf{Model-Predictive Control} [$\textsf{MPC}$]: Runs Algorithm~\ref{alg:mpc} with prior $\beta_{1} = \mathbf{0},\Sigma_{1} = I$, uses samples of $X_{i}$ from the first batch and uses batch sizes $\bar{n}_{t} = N\lambda_{t}$.
 \item \textbf{Model-Predictive Control (Noisy)} [$\textsf{MPC  (noisy)} $]: Same as \textsf{MPC}, but uses noisy predictions of arrival rates $\widehat{n}_{t}=N\hat{\lambda}_{t}$ where $\hat{\lambda}_{t} \sim \text{Dirichlet}_{K\lambda}(\cdot)$.
\end{itemize}
We also benchmark these uniform exploration strategies with a non-uniform exploration policy.
\begin{itemize}
\item \textbf{Batched Thompson Sampling} [\textsf{TS}]~\cite{kalkanli2021batched, karbasi2021parallelizing}: At each period $t$, it samples item embeddings from the posterior  $\theta_{t} \sim N(\beta_{t},\Sigma_{t})$ and assigns items to each user in the batch according to $A_{i} = \arg \max_{a\in\mathcal{A}} X_{i}^{\top}\theta_{t,a}$. It then uses all the batch data to update the posterior mean and covariance.
\end{itemize}
\begin{table*}[t]
\scriptsize

$K = 10$ items 
\vspace{0.1cm}

\begin{tabular}{lcccccc|cccccc}
\toprule
 & \multicolumn{6}{c|}{MovieLens-1M} & \multicolumn{6}{c}{Netflix} \\
\midrule
$N$ samples & \multicolumn{3}{c}{500} & \multicolumn{3}{c|}{5000} & \multicolumn{3}{c}{500} & \multicolumn{3}{c}{5000} \\
\midrule
Arrival $\lambda$ & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike & Constant & Increasing & Spike \\
\midrule
\textsf{EpsGreedy}$^{*}$ & 0.456 & 0.494 & 0.511 & 0.227 & 0.232 & 0.267 & 0.197 & 0.225 & 0.243 & 0.127 & 0.133 & 0.144 \\
\textsf{TheoryETC}$^{*}$ & 0.349 & 0.350 & 0.373 & \textbf{0.158} & 0.167 & 0.170 & \textbf{0.159} & 0.169 & \textbf{0.171} & \textbf{0.075} & 0.092 & 0.087 \\
\textsf{SimpleETC}       & \textbf{0.278} & 0.436 & \textbf{0.306} & \textbf{0.157} & 0.130 & \textbf{0.130} & 0.168 & 0.228 & 0.192 & \textbf{0.075} & 0.102 & \textbf{0.082} \\
\midrule
\textsf{Planner}         & \textbf{0.280} & 0.411 & \textbf{0.305} & \textbf{0.157} & 0.130 & \textbf{0.130} & 0.168 & 0.170 & 0.191 & \textbf{0.075} & 0.102 & \textbf{0.082} \\
\textsf{Planner (noisy)} & 0.286 & 0.341 & \textbf{0.307} & \textbf{0.157} & 0.130 & \textbf{0.130} & 0.164 & 0.165 & 0.178 & \textbf{0.075} & 0.100 & \textbf{0.082} \\
\textsf{MPC}             & 0.285 & \textbf{0.326} & \textbf{0.308} & \textbf{0.157} & \textbf{0.126} & \textbf{0.130} & 0.169 & 0.163 & \textbf{0.171} & \textbf{0.074} & \textbf{0.081} & \textbf{0.081} \\
\textsf{MPC (noisy)}     & \textbf{0.282} & 0.350 & \textbf{0.305} & \textbf{0.157} & \textbf{0.125} & \textbf{0.130} & 0.165 & \textbf{0.158} & \textbf{0.167} & \textbf{0.074} & 0.087 & \textbf{0.081} \\
\bottomrule
\end{tabular}

\caption{\label{table:min_explore} Average regret for uniform exploration policies across contextual bandit settings with $K = 10$, where the exploration rate is constrained $\eps_{t}\geq0.05$ for all $t$. \textsf{Planner} and \textsf{MPC}, which incorporate the constraint into the optimization problem, reduce their exploration in the beginning as a response and more closely resemble \textsf{SimpleETC}.}
\end{table*}




\paragraph{Results}

Table~\ref{table:experiments} displays the average regret for each policy across different datasets and settings. We see that even when fixing the same total sample size $N$ for the horizon (in expectation), the distribution of arrivals $\lambda$ across periods has a large impact on regret and the optimal exploration strategy. Despite its simplicity, we find that \textsf{SimpleETC} often outperforms \textsf{TheoryETC}$^{*}$ for the Constant arrival pattern as well as the Spike arrival pattern (when $N = 5000$), despite the latter method's theoretical justification (and the grid search over optimal constants). For the Spike pattern, the batch size arriving on period $t = 2$ is large enough that it is better to be greedier at $t = 2$, even if this results in less data collected for future periods. However, \textsf{SimpleETC} is ineffective for the Increasing pattern because the first batch is too small to learn an effective policy and the strategy does not explore in future periods. This illustrates that under batched feedback, the optimal strategy can depend sensitively on the distribution of batch sizes, which makes it difficult to reason from first principles.

On the other hand, we observe that the optimization-based algorithms \textsf{Planner} and \text{MPC} are able to automatically tailor exploration to the structure of the batches. The exploration schedules consistently match and even outperform \textsf{SimpleETC} and \textsf{TheoryETC}$^{*}$ \emph{uniformly} across patterns, applying the strategy most appropriate to the situation. These algorithms do not overfit either; even under very noisy estimates of the true arrival pattern, both \textsf{Planner (noisy)} and \text{MPC (noisy)} achieve only slight worse performance. The consistent performance of this policy is promising for practitioners, as they can use the same algorithm for different settings, instead of having to know beforehand what the appropriate exploration strategy is. And when constraints are introduced, such as a minimum exploration rate of $\eps_{t}\geq 0.05$ in Table~\ref{table:min_explore}, incorporating these constraints into the optimization problem~\eqref{eqn:opt} induces less exploration in the beginning to account for this, delivering similar or better performance to the best heuristic in each setting. We also see that \textsf{MPC} often achieves lower regret than the static \textsf{Planner}, showing that adjusting the exploration rate during the horizon helps correct for any planning errors.

Finally, we note that surprisingly, the simple uniform exploration policies we consider consistently outperform Thompson Sampling in these batched, short-horizon settings. We find that Thompson Sampling suffers from over-exploration, which has also been observed in other works~\cite{jin2023thompson, do2024epsilon}. One driver of over-exploration is that Thompson Sampling lacks awareness of the time horizon, and explores until the posterior converges which may be sub-optimal for short time horizons. We do indeed find that time horizon is longer and when the arrival pattern is Constant, the performance gap closes. This illustrates though that seemingly simple and sub-optimal uniform exploration strategies can be surprisingly effective in settings relevant for practitioners.



% \vspace{0.2cm}
% \begin{tabular}{lccccccccc}
% \toprule
% \multicolumn{10}{c}{10 Items, $s^{2} = 25$} \\
% \midrule
% Num Samples & \multicolumn{3}{c}{500} & \multicolumn{3}{c}{1000} & \multicolumn{3}{c}{5000} \\
% \midrule
% Pattern & frequent & increasing & spike & frequent & increasing & spike & frequent & increasing & spike \\
% \midrule
% \textsf{EpsGreedy}$^{*}$ & 1.048 & 1.063 & 1.120 & 0.837 & 0.925 & 0.928 & 0.663 & 0.643 & 0.672 \\
% \textsf{TheoryETC}$^{*}$ & 1.242 & 1.230 & 1.228 & 1.018 & 1.038 & 1.033 & 0.618 & 0.637 & 0.632 \\
% \textsf{SimpleETC} & 0.811 & 1.122 & 1.034 & \textbf{0.844} & 0.832 & 0.773 & \textbf{0.390} & 0.788 & 0.431 \\
% \midrule
% \textsf{Planner} & 0.807 & 0.912 & 1.035 & \textbf{0.844} & 0.845 & 0.773 & \textbf{0.391} & 0.788 & 0.431 \\
% \textsf{Planner (noisy)} & 0.843 & \textbf{0.846} & 0.987 & \textbf{0.847} & \textbf{0.710} & 0.763 & 0.391 & 0.770 & 0.431 \\
% planner & \textbf{0.735} & 0.894 & \textbf{0.930} & 0.858 & \textbf{0.716} & \textbf{0.742} & 0.390 & \textsf{0.573} & \textsf{0.427} \\
% est\_planner & 0.791 & 0.870 & \textbf{0.928} & \textbf{0.837} & \textbf{0.719} & 0.777 & 0.388 & 0.617 & \textsf{0.428} \\

% \bottomrule
% \end{tabular}

==> mpc.tex <==
\section{Differentiable Bayesian Regret}
\label{sec:mpc}



Ideally, we could select the exploration rates $\eps_{1:T}$ to directly minimize $\text{Regret}_{T}(\eps_{1:T})$ in~\eqref{eqn:eps_regret}. However, there are two issues that make $\text{Regret}_{T}(\eps_{1:T})$ unsuitable for optimization. First, $\text{Regret}_{T}(\eps_{1:T})$ depends on the unknown item embeddings $\theta$ through the reward 
model $r(x,a)$. Second, quantifying the benefit of exploration requires precisely understanding how additional samples will affect the greedy policy in future periods, which is difficult to characterize and does not have a simple closed form that can be optimized. In general, it is well-known that regret  is a difficult objective to directly optimize, which is why existing algorithmic principles such as UCB or Thompson Sampling rely on optimizing proxies or upper bounds of regret instead (e.g. Hoeffding Bound)~\cite{lattimore2020bandit}. However, in this section, we show that \emph{Bayesian regret} does not suffer from these two issues and is amenable to optimization.

We assume the platform has a prior distribution over the unknown item embeddings:
\begin{align}
\theta \sim N(\beta_{1}, \Sigma_{1})
\end{align}
where $\beta_{1}\in \R^{Kd}$ and $\Sigma_{1} \in \R^{Kd \times Kd}$ are the prior mean and covariance of the item embeddings. Typically, $\beta_{1} = \mathbf{0}$ and $\Sigma = \sigma^{2}\mathbf{1}$ for some $\sigma^{2}>0$, although the prior could be calibrated to the statistics of existing item embeddings. 

We introduce three assumptions that enable simplify the structure of the Bayesian posterior updates. First, We assume Gaussian noise, as this implies that the posterior distribution of $\theta$ is also Gaussian with closed-form expressions for the posterior mean and covariance. 
\begin{assumption}
\label{ass:normal}
The noise $\eta_{i}$ are distributed iid and are normally distributed $N(0,s^{2})$.
\end{assumption}
We also assume that posterior updates only use data from the `explore' group:
\begin{assumption}
\label{ass:explore_only}
The posterior is updated using only data from the `explore' group, i.e. the history we are conditioning on $H_{t} = \sigma(\cup_{s=1}^{t-1}\mathcal{D}_{s})$ where $\mathcal{D}_{s} = \cup_{i=1}^{n_{s}}\{(X_{i},A_{i},R_{i},\xi_{i}):\xi_{i}=1\}$.
\end{assumption}
One limitation of this assumption is that it ignores data gathered by the greedy policy. Nevertheless this captures the exploration-exploitation tradeoff and reflects practical implementations, which typically only use randomly sampled data to train the policy. 



Our final assumption is that the prior covariance $\Sigma_{1}$ is block-diagonal across items. 
\begin{assumption}
\label{ass:block}
We assume that the prior covariance is of the form:
    $$\Sigma_{1} = \mathbf{diag}(\Sigma_{1,1},\ldots \Sigma_{1,a}, \ldots, \Sigma_{K,a})$$
where $\Sigma_{1,a} \in \R^{d\times d}$ for all $a\in \mathcal{A}$.
\end{assumption}
We do not need this assumption for the validity of Bayesian updating, but it simplifies notation by allowing for the posterior to be updated independently for each item.

Under these assumptions, we obtain a standard expression for the posterior distribution of $\theta$ at the beginning of period $t$. The posterior distribution of $\theta$ given $H_{t}$ follows a normal distribution:
\[
\theta|H_{t} \sim N(\beta_{t},\Sigma_{t})
\]
where the posterior mean $\beta_{t}$ and covariance $\Sigma_{t}$ follow the recursive formula for each $a$:
\begin{align}
    \Sigma_{t+1,a} &= \left( \Sigma_{t,a}^{-1} + I_{t,a}(\eps_{t}) \right)^{-1} \label{eqn:true_sigma_update}\\
    \beta_{t+1,a} &= \Sigma_{t+1,a}\left( \Sigma_{t,a}^{-1} \beta_{t} + I_{t,a}(\eps_{t})^{-1} \left(\sum_{i=1}^{n_{t}}  \xi_{i}\mathbf{1}\{A_{i} = a\}R_{i}X_{i} \right) \right) \label{eqn:true_beta_update}\\
    I_{t,a}(\eps_{t})  & \equiv s^{-2}\sum_{i=1}^{n_{t}}\xi_{i}\mathbf{1}\{A_{i} = a\}X_{i}X_{i}^{\top} \label{eqn:stoch_design}
\end{align}
% where $X_{i}\stackrel{iid}{\sim}\mu$, $\xi_{i}\stackrel{iid}{\sim}\text{Ber}(\eps_{t})$, and $A_{i}\stackrel{iid}{\sim}\text{Multinomial}(\mathbf{1}/K)$ and all are independent of each other.

% We denote $(\beta_{t}, \Sigma_{t})$ to be the posterior parameters at period $t$ and before observing the data from batch $t$, and let $\beta_{t,a} \in \R^{d}$ and $\Sigma_{t,a}\in \R^{d\times d}$ denote the posterior parameters for each item $a$. 
We use the notation $\E_{1}$ to denote expectation of $\theta$ under the prior and $\E_{t}[\cdot]\equiv \E[\cdot |H_{t}]$ to denote expectation under the posterior at period $t$ so,
\begin{align}
    \E_{t}[r(x,a)]= x^\top \E_{t}[\theta_{a}]=x^\top \beta_{t,a}
\end{align}
% The posterior distribution of $\theta$ is also normally distributed. Consider a fixed sequence $\eps_{1:T}$. We denote $(\beta_{t}, \Sigma_{t})$ to be the posterior parameters at period $t$ and before observing the data from batch $t$. Starting from $(\beta_{t}, \Sigma_{t})$, the posterior update using data $(X_{i}, A_{i}, R_{i})$ drawn from the explore group at batch $t$ is as follows:

% where $\xi\in \{0,1\} \sim \text{Bern}(\eps_{t})$ indicates whether $i$ is in the explore group and $I_{n,t}(\eps_{t})$ is the (sampled) design matrix from the explore group after with rate $\eps_{t}$. 

An important property of the Bayesian linear regression model for optimization is the existence of closed-form expressions for the distribution of \emph{future} posterior states, conditional on the current posterior and a fixed exploration rate. A derivation can be found in~\cite{che2024optimization}.

\begin{lemma}~\cite{che2024optimization}
\label{lemma:posterior}
Suppose Assumptions~\ref{ass:normal}-\ref{ass:block} hold. Consider any exploration rates $\eps_{1:T}$, and any $1\leq t\leq s$. For each item $a$, the distribution of the posterior $(\beta_{s,a}, \Sigma_{s,a})$, conditional on the period $t$ posterior $(\beta_{t,a}, \Sigma_{t,a})$ is given as follows:
\begin{align}
    \Sigma_{s,a} &\stackrel{d}{=} \left( \Sigma_{t,a}^{-1} +  \sum\nolimits_{l=t}^{s-1}I_{t,a}(\eps_{t}) \right)^{-1} \label{eqn:pred1}\\
    \beta_{s,a} &\stackrel{d}{=} \beta_{t,a} + (\Sigma_{t,a} - \Sigma_{s,a})^{1/2}Z_{s} \label{eqn:pred2}
\end{align}
where $Z_{t} \sim N(0,I)$ is a standard Gaussian random vector and $I^{a}_{n,s}$ is the empirical design matrix given by~\eqref{eqn:stoch_design} with $X_{i}\stackrel{iid}{\sim}\mu$ ($\mu$ is the distribution of user embeddings), $\xi_{i}\stackrel{iid}{\sim}\text{Ber}(\eps_{s})$, $A_{i}\stackrel{iid}{\sim}\text{Multinomial}(\mathbf{1}/K)$.
\end{lemma}
Lemma~\ref{lemma:posterior} captures how future posterior beliefs will change based on the exploration rates. Setting a high exploration rate $\eps_{t}$ induces a larger update in future beliefs while a low exploration rate will not change future beliefs from the current posterior. Thus, the lemma precisely measures the \emph{value of exploration} not only for the next period but for every future period in the time horizon, and doing so only requires sampling from a standard normal distribution.

We now turn to the Bayesian regret objective, which is more amenable to optimization as it does not depend on unknown item embeddings. Instead, it averages regret~\eqref{eqn:eps_regret} over item embeddings drawn from the prior distribution:
\begin{align}
& \min_{\eps_{1:T}}   \E_{\theta \sim N(\beta_{1},\Sigma_{1} )}\left[\text{Regret}_{T}(\eps_{1:T}) \right] \label{eqn:bayes_eps_regret}\\
&=\min_{\eps_{1:T}}
\sum_{t=1}^{T} n_{t} \E_{1}[
\eps_{t}\text{Reg}(X_{i}, \mathbf{1}/K)  
     + (1-\eps_{t})\text{Reg}(X_{i}, \widehat{\pi}_{t})]
\end{align}
where the expectation in the second line denotes expectation over $X_{i}\sim \mu$, $\xi_{i} \sim \text{Ber}(\eps_{i})$, random sampling $A_{i}$, and the prior distribution of $\theta$. One benefit of the Bayesian model is that Regret can be written in closed form in terms of prior and posterior parameters. To illustrate, we first look at the regret of the greedy policy $\text{Reg}(X_{i}, \widehat{\pi}_{t})$. Given the Bayesian formulation, we slightly revise the definition of the greedy policy $\hat{\pi}_{t}$: it assigns the item that maximizes expected reward at period $t$,
\begin{align}
    \hat{\pi}_{t}(a|x)& \equiv
    \mathbf{1}\{ a = \arg\max_{a} \E_{t}[r(X_{i},a)]\} \label{eqn:bayes_greedy} \\
    &=\mathbf{1}\{ a = \arg\max_{a} X_{i}^{\top}\beta_{t,a}\}.  \nonumber
\end{align}

We arrive at our main result, which gives a concrete expression for Bayesian regret.
\begin{proposition}
\label{thm:diff_regret}
Under Assumptions~\ref{ass:normal}-\ref{ass:block}, Bayesian regret~\eqref{eqn:bayes_eps_regret} under the uniform exploration policy with the greedy assignment given by~\eqref{eqn:bayes_greedy} is equal to 
\begin{align}
&\E_{1}[\text{Regret}_{T}(\eps_{1:T})]  \nonumber \\
&= n\E_{1}[r^{*}(X_{i})]-
\sum_{t=1}^{T}
n_{t}
\E\left[\eps_{t} X_{i}^{\top}\bar{\beta}_{1} + (1-\eps_{t})\max_{a}X_{i}^{\top}\beta_{t,a}\right] \label{eqn:diff_regret}
\end{align}
where $\bar{\beta}_{1} = \sum_{k=1}^{K} \beta_{1,a}$ and for all items $a\in \mathcal{A}$,
\begin{align}
\Sigma_{t,a}^{-1} &= \Sigma_{1,a}^{-1} +  \sum\nolimits_{l=1}^{t-1}I_{l,a}(\eps_{l})
\label{eqn:sigma_update}
\\
    \beta_{t,a} &= \beta_{1,a} + (\Sigma_{1,a} - \Sigma_{t,a})^{1/2}Z_{t} 
    \label{eqn:beta_update}
\end{align}
where $I_{t,a}(\eps_{t})$ is defined in~\eqref{eqn:stoch_design} and the expectation in~\eqref{eqn:diff_regret} is over $Z_{t}\stackrel{iid}{\sim}N(0,I)$, $X_{i}\stackrel{iid}{\sim}\mu$, $\xi_{i}\stackrel{iid}{\sim}\text{Ber}(\eps_{s})$, and $A_{i}\stackrel{iid}{\sim}\text{Multinomial}(\mathbf{1}/K)$.
\end{proposition}

See proof in Section~\ref{sec:appendix}. Proposition~\ref{thm:diff_regret} provides an exact expression for Bayesian regret, which can be efficiently estimated through Monte Carlo simulation of standard random variables based on known information. It presents a precise characterization of the exploration-exploitation trade-off -- a higher $\eps_{t}$ reduces immediate reward by placing more weight on randomization, but increases future reward by increasing the variance of future posteriors $\beta_{t,a}$ (i.e. inducing a larger posterior update), which increases the expected reward from the greedy policy in the future $\E_{1}[\max_{a}X_{i}^\top \beta_{t,a}]$. 
% And unlike existing approaches in the contextual bandit literature, this is an exact characterization of regret for any $n$ and batching scheme $n_{t}$ and does not invoke proxies or upper bounds, and only relies on standard assumptions for Bayesian bandits.

Still, the expressions~\eqref{eqn:sigma_update}-\eqref{eqn:beta_update} are difficult to directly optimize because $I_{t,a}(\eps_{t})$ depends on $\eps_{t}$ through the realizations of Bernoulii r.v.s. $\xi_{i}$. Nevertheless, when $n_{t}$ is large the dependence of $I_{t,a}$ on $\eps_{t}$ simplifies, as a consequence of the Law of Large Numbers (applied to each entry of the matrix). If $\E_{\mu}[\|X_{i}\|^{4}] < \infty$, then with probability 1,
% \begin{lemma}
% For all $t\leq T$ and $a\in \mathcal{A}$, as $n_{t}\to \infty$, we have that with probability 1
\begin{align}
    \|n_{t}^{-1}I_{t,a}(\eps_{t}) - \eps_{t}I \|_{\infty} \to 0
\end{align}
where $I$ is the population design matrix.
\begin{align}
\label{eqn:design}
\mathcal{I}\equiv s^{-2}K^{-1}\E_{X_{i}\sim\mu}[X_{i}X_{i}^{\top}]
\end{align}
Considering that large batch sizes $n_{t}$ are common in practice, this motivates the approximation of the empirical design matrix with the considerably simpler population design matrix:
\begin{align}
I_{t,a}(\eps_{t}) \approx n_{t}\eps_{t}\mathcal{I}
\end{align}
% Applying this approximation to~\eqref{eqn:sigma_update}, we obtain our differentiable approximation to Bayesian regret:
% \begin{align}
% n\E_{1}[r^{*}(X_{i})]-
% \sum_{t=1}^{T}
% n_{t}
% \E\left[\eps_{t} X_{i}^{\top}\bar{\beta}_{1} + (1-\eps_{t})\max_{a}X_{i}^{\top}\beta_{t,a}\right]
% \end{align}
% where
% \begin{align}
% \Sigma_{t,a} &= \left( \Sigma_{1,a}^{-1} +  \sum\nolimits_{l=1}^{t-1}\eps_{t}n_{t}I \right)^{-1}
% \label{eqn:sigma_update}
% \\
%     \beta_{t,a} &= \beta_{1,a} + (\Sigma_{1,a} - \Sigma_{t,a})^{1/2}Z_{t} 
%     \label{eqn:beta_update}
% \end{align}
We substitute into~\eqref{eqn:sigma_update} to obtain the following approximation for the update for $\Sigma$:
\begin{align}
\label{eqn:diff_sigma_update}
\Sigma_{t,a}^{-1} &= \Sigma_{1,a}^{-1} +  \sum\nolimits_{l=1}^{t-1}\eps_{l}n_{l}\mathcal{I}
\end{align}
Replacing~\eqref{eqn:sigma_update} with the approximation~\eqref{eqn:diff_sigma_update} makes the Bayesian regret~\eqref{eqn:diff_regret} differentiable in $\eps_{t}$, as $\Sigma_{t},\beta_{t}$ are differentiable in $\eps_{t}$ under any realization of $Z_{t}$ and regret is differentiable in $\beta_{t}$. This approximation also makes it easier to simulate and only requires samples of $Z_{t}\stackrel{iid}{\sim}N(0,I)$, $X_{i}\stackrel{iid}{\sim}\mu$.
